Matryoshka: Stealing Functionality of Private ML Data by Hiding Models in Model

In this paper, we present a novel insider attack called Matryoshka, which employs an irrelevant scheduled-to-publish DNN model as a carrier model for covert transmission of multiple secret models which memorize the functionality of private ML data stored in local data centers. Instead of treating the parameters of the carrier model as bit strings and applying conventional steganography, we devise a novel parameter sharing approach which exploits the learning capacity of the carrier model for information hiding. Matryoshka simultaneously achieves: (i) High Capacity -- With almost no utility loss of the carrier model, Matryoshka can hide a 26x larger secret model or 8 secret models of diverse architectures spanning different application domains in the carrier model, neither of which can be done with existing steganography techniques; (ii) Decoding Efficiency -- once downloading the published carrier model, an outside colluder can exclusively decode the hidden models from the carrier model with only several integer secrets and the knowledge of the hidden model architecture; (iii) Effectiveness -- Moreover, almost all the recovered models have similar performance as if it were trained independently on the private data; (iv) Robustness -- Information redundancy is naturally implemented to achieve resilience against common post-processing techniques on the carrier before its publishing; (v) Covertness -- A model inspector with different levels of prior knowledge could hardly differentiate a carrier model from a normal model.

==> tex/alg/fill.tex <==
\begin{algorithm}
 \caption{The \textbf{Fill}($P$, $f$, $v$) Primitive}
 \label{alg:fill}
  {\fontsize{10}{10}\selectfont
 \begin{algorithmic}[T]
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \REQUIRE $P = P_w \cup P_b \cup P_s$ (an initialized ParamPool), $f$ (a DNN model), $v$ (an integer secret).
 \ENSURE $\mathcal{P}(\cdot, v)$ (a hash map).
 \\
  \STATE $v_w, v_b, v_s \gets v \mod |P_w|, v \mod |P_b|, v \mod |P_s|$
  {\small{\hskip3em$\vartriangleright$ Derivation of initial random shift on each parameter group.}}
 \\ 
%  \STATE {Generate a random permutation $\pi_w$ ($\pi_b, \pi_s$) of integers from 0 to $|P_w|$  ($|P_b|, |P_s|$) with seeds $v_w (v_b, v_s)$.}
% \STATE {$\pi_w, \pi_b, \pi_s \gets $RandPerm($|P_w|,v_w$), RandPerm($|P_b|, v_b$), RandPerm($|P_s|, v_s$)}
%  {\small{\hskip3em$\vartriangleright$ Generate a random permutation $\pi_w$ ($\pi_b, \pi_s$) of integers from 0 to $|P_w|$  ($|P_b|, |P_s|$) with seeds $v_w (v_b, v_s)$.}}\\
\STATE Generate a random permutation $\pi_w$ ($\pi_b, \pi_s$) of integers from 0 to $|P_w|$  ($|P_b|, |P_s|$) with seeds $v_w (v_b, v_s)$.\\
%   \STATE Generate a random element $\pi_w$ ($\pi_b, \pi_s$) from the permutation group on $|P_w|$  ($|P_b|, |P_s|$) with seeds $v_w (v_b, v_s)$. \\ 
 \STATE  $\mathcal{P}(\cdot, v) \gets \{\}$ {\small{\hskip1em$\vartriangleright$ Initialize a hash map to store the mapping relation.}} \\
% \STATE $i_w\gets 0, i_b\gets 0, i_s \gets 0$
  \FOR {each scalar parameter $w$ in $f$}
  \IF{$w$ belongs to a \{weight, scale, bias\} parameter}
  \SWITCH{$\text{type}(w)$}
  \CASE{weight}
   \STATE {$w_P \gets (\pi_w \circ P_w)[v_w]$, $v_w \gets (v_w + 1)$ mod $|P_w|$}
%   \IF {$i_w == |P_w|$}
    % $v_w \gets v_w + 1$,
    % $\pi_w \gets $RandPerm($|P_w|,v_w$)
% \ENDIF
  \ENDCASE
    \CASE{bias}
   \STATE  {$w_P \gets (\pi_b \circ P_b)[v_b]$, $v_b \gets (v_b + 1)$ mod $|P_b|$} 
%   \IF {$i_b == |P_b|$}
%     $v_b \gets v_b + 1$,
%     $\pi_b \gets $RandPerm($|P_b|,v_b$)
% \ENDIF
  \ENDCASE
    \CASE{scale}
   \STATE {$w_P \gets (\pi_s \circ P_s)[v_s]$, $v_s \gets (v_s + 1)$ mod $|P_s|$}
%   \IF {$i_w == |P_w|$}
%     $v_s \gets v_s + 1$,
%     $\pi_s \gets $RandPerm($|P_s|,v_s$)
% \ENDIF
  \ENDCASE
  \ENDSWITCH
    \STATE{$w$.data $\gets w_P$.data} \\
    \STATE{$\mathcal{P}(\cdot, v)$.Add($w\to{w_P}$)}   \\ 

  \ELSE
  \STATE{CONTINUE}
  \ENDIF
  \ENDFOR
  \RETURN $\mathcal{P}(\cdot, v)$
 \end{algorithmic}}
 \end{algorithm}

==> tex/data_hiding_repo.tex <==
 
 %%%%%%%%%%%%%%%%%%%%%
 
%%%% 
\subsection{Effectiveness of Data Stealing}
\label{sec:exp:data_stealing}
Next, we present evaluation results on stealing a sensitive subset of data inputs with Matryoshka. Specifically, we conduct data stealing on two image datasets of increasing resolultion (i.e., CIFAR-10 and FaceScrub \cite{Ng2014ADA}), and an audio dataset (Google's Speech Command \cite{Warden2018SpeechCA}). We randomly sample $M$ target inputs from the dataset as the sensitive targets, and use the ResNet-18 on CIFAR-10 as the carrier model. For baselines, we also compare Matryoshka with three conventional data hiding techniques, namely, \textit{LSB}, \textit{Sign} and \textit{Covariance} \cite{Song2017MachineLM}. The three bsaelines utilize the least-significant bits, the sign and the covariance between model parameters and the sensitive data for information hiding. Fig.\ref{fig:data_stealing} reports the SSIM of the reconstructed images and the accuracy of the carrier model when the $M$ increases from $8$ and $1024$ on Facescrub, a dataset composed of celebrity face images of resolution $224\times{224}$. The omitted results on other two datasets are presented in Appendix \ref{sec:appendix:exp}.  
 

%%%%%%%%%%%%% BEGIN OF Facescrub dataset
\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.45\textwidth]{img/ssim_bar_face.pdf}
\vspace{-0.2in}
\caption{The effectiveness of data stealing in terms of SSIM and the accuracy of the carrier model when the number of target inputs continually increases on FaceScrub. }
\label{fig:data_stealing}
\end{center}
\vspace{-0.3in}
\end{figure}
%%%%%%%%%%%%%% END OF FaceScrub dataset


\noindent\textbf{Results \& Analysis.} As Fig.\ref{fig:data_stealing} shows, Matryoshka can steal over $1000$ face images with an SSIM uniformly higher than $0.97$ and with less than $1\%$ accuracy loss on the carrier model. This substantially surpasses the performance of existing data hiding techniques. On the one hand, in the upper part of Fig.\ref{fig:data_stealing}, the corresponding result for Sign, Covariance and LSB is unable to be derived when $N$ reaches $64, 128$ and $1024$ respectively. It is mainly because, when the number of target inputs hits such a size, either the information capacity in the sign bit, the covariance, or the bits can no longer afford the required capacity for hiding all the images (i.e., about $147$MB, $3\times$ of a ResNet-18), which directly inhibits the baselines from being executed. In contrast, based on parameter sharing instead of directly modifying the parameter for data hiding, Matryoshka has no hard upper limit on its hiding capacity and is more flexible to more general data stealing scenarios. On the other hand, our proposed attack achieves the optimal SSIM compared with both the Sign and the Covariance encoding. Although the SSIM of LSB remains $1$, it drastically decreases the performance of the carrier model when the number of inputs is no smaller than $256$. For example, when $N=256$, the LSB encoding has to totally modify the last $24$ bits of all the 32-bit parameters in ResNet-18 to afford the required capacity, which degrades the carrier model to a totally random model (i.e., ACC=$10\%$). In comparison, the carrier model in Matryoshka preserves most of its utility. Besides, the detection and the obfuscation of LSB encoding is a long-standing topic in steganalysis \cite{Provos2003HideAS}, while, for Matryoshka, both remain open problems for future mitigation research (\S\ref{sec:exp:resilience} \& \S\ref{sec:evasion}).  For better intuition, we also qualitatively compare the results of our attack with Covariance and Sign encoding in Fig.\ref{fig:facescrub_visualization} when stealing $8$ random data samples from FaceScrub. As is shown, our reconstructed images (i.e., the 3rd row) are almost perceptually indistinguishable with the ground-truth ones, which highly conforms to our quantitative results in terms of SSIM.  

%%%%%%%%%%%%% BEGIN OF Facescrub visualization
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.45\textwidth]{img/facescrub_visualize.jpg}
\caption{Sampled results on Facescrub with different data stealing approaches.}
\label{fig:facescrub_visualization}
\end{center}
\vspace{-0.3in}
\end{figure}
%%%%%%%%%%%%%% END OF FaceScrub visualization


 Besides, we measure the effectiveness of memorization-oriented stealing by the pairwise difference between the reconstructed and ground-truth samples. For image data, we follow \cite{wang2004image} to use the \textit{structural similarity index} (SSIM) as the metric. A higher SSIM implies more effective data stealing. For audio data, we use the \textit{mean square error} (MSE) as the metric. More details can be found in Appendix \ref{sec:appendix:exp}.



\noindent\textbf{Memorization-Oriented 
Stealing.} 
For stealing a subset of sensitive inputs, i.e., $\{x_i\}_{i=1}^{M_k}$, from a private dataset, we propose to model the secret learning task in the supervised learning framework. Specially, we aim at training a generator-like architecture $f_k$ which maps noise vectors from a predefined noise space $Z$ to each one of the sensitive inputs. By choosing a common noise distribution $\mathcal{N}_k$ on $Z$ and a secret integer $s_k \in \mathbb{N}_{+}$, the attacker samples a sequence of noise vectors $z_1, z_2, \hdots, z_{M_k} \sim \mathcal{N}_k$ when the random seed is specified as $s_k$. By pairing the noise vector and the sensitive inputs as $\{(z_i, x_i)\}_{i=1}^{M_k} (:=\tilde{D}_k)$, the attacker constructs the secret learning task below for sensitive data stealing
\begin{equation}
    \min_{\theta_k}L_k(\theta_k) := \frac{1}{|\tilde{D}_k|}\sum_{(z_i, x_i)\in\tilde{D}_k}d(f_k(z_i;\theta_k), x_i),
\end{equation}
where $d$ is a distance metric defined on the input space. As pseudorandomness is machine-independent in most popular DL frameworks and operating systems \cite{pytorch_random,Matsumoto1998MersenneTA}, the colluder can deterministically replicate the noise sequence after knowing the specific noise distribution and the integer seed $s_k$. Unlike directly encoding sensitive inputs in model parameters \cite{Song2017MachineLM}, our approach addresses the data heterogeneity problem in existing attacks by converting data hiding to model hiding. As models are distributionally homogeneous (\S\ref{sec:pilot_study}), our approach substantially improves the hiding capacity while preserving the normal utility of the carrier model (\S\ref{sec:exp:data_stealing}).   %% discussion of the difference

Otherwise, for the $k$-th target dataset, the attacker uses the securely communicated knowledge of the fixed distribution and the integer random seed to replicate the set of random noise vectors $z_1, \hdots, z_{M_k}$. Finally, he/she dumps each $f_k(z_i)$ for approximately recovering the sensitive  input $x_i$. 


% Table \ref{tab:datasets} summarizes the basic information of the datasets, tasks, architectures and the perofmrance metrics used in our evaluation. 

==> tex/orphanage.tex <==
In these cases, either the functionality or the sensitive part of the dataset is under leakage. 


%%%%% SOME REDUNDANT DETAILS IN THE ATTACK OVERVIEW 
    Specifically, (i) if the attacker wants to steal the functionality of a private dataset $D_k := \{(x_i, y_i)\}_{i=1}^{M_k} \subset {\mathcal{X}_i}\times\mathcal{Y}_i$ used for supervised learning, he/she chooses an architecture $f_k:\mathcal{X}_i \to \mathcal{Y}_i$ with a corresponding loss function $\ell_{k}$. In this case, the training dataset for the attacker is exactly $\tilde{D}_k = D_k$. (ii) Otherwise, if the target dataset $D_k := \{x_i\}_{i=1}^{M_k}$ is for unsupervised learning or the attacker is more curious about the sensitive inputs in a supervised learning task, he/she is recommended to implement $f_k$ as a generator-like architecture (e.g., DCGAN \cite{Radford2016UnsupervisedRL}), which maps a high-dimensional noise vector to the input space $\mathcal{X}_i$. To prepare the training set for $f_k$, the attacker selectively chooses the subset of private data he/she wants to leak, and pair each sensitive data input $x_i$ with a noise vector $z_i$. To reduce the information which is required to be colluded on, the set of noise vectors is sequentially generated under a fixed integer seed from a secret distribution whose configuration is exclusively known to the insider and the colluder. For simplicity, we denote the training set for the attacker as $\tilde{D}_k = \{(z_i, x_i)\}_{i=1}^{M_k}$ (with a slight abuse of the symbol $M_k$). In this case, we choose the loss function $\ell_k$ as the mean square error.
    
      

\subsubsection{On Random Perturbation}
Finally, we evaluate the performance of secret models when a white noise is added uniformly to the parameters of the carrier model. 


\noindent\textbf{(2) Filter Pruning} (FP): Different from the granularity of weight pruning, we set the values of a $\beta$ proportion of filters with the smallest L2 norm as $0$ \cite{Li2017PruningFF}. For the above two pruning techniques, we vary $\beta$ from $0.1$ to $0.9$ in our experiments.  


%%%%%%%%%%%% RELATED WORK ABOUT MODEL COMPRESSION
%%%%%%%% Hiding (or Training) Models in Model
During these years, several works attempt to turn the over-parameterization of DNNs into strengths for different scenarios by sharing weights across disparate models with the same or similar architectures. For example, to diminish the catastrophic forgetting, Cheung et al. propose to perform multiple tasks in the same parameters of a neural network by storing the weights of each task via superposition. Based on [], Cai et al. propose a new methodology to train a large number of sub-networks within the same weight set to satisfy the accuracy and efficiency constraints under various hardware platforms. Different from our work, the multiple tasks considered in [] are closely related (e.g., image classification with different data distribution in continue learning) and the sub-networks in [] with elastic depth and width are designed for the same task.

This mechanism above can be further applied to undermine the intellectual property of the proprietary model. Guo et al. introduce a novel steganographic technique to embed a proprietary model into a carrier model intended for public release by permuting the weights layer by layer with a secret key. The secret model, however, is limited to retaining the same architecture and targeted for the closely related task with the carrier model, while Matryoshka can hide several models with totally different architectures (e.g. ResNet, MobileNetv1-SSD, TextCNN, et al.) for each specific task (e.g. object detection, text or audio classification) into only one carrier model, which poses severe privacy leakage threat to the proprietary secret models or the unexposed data.

% Appendix \ref{sec:appendix:dnn} presents more details on parameter initialization and batch normalization.    


%% This paragraph justifies why stealing private ML datasets is meaningful and threatening
\subsubsection{Privatization of ML Datasets} Although there are supportive voices calling for a future of open ML data \cite{hai_report}, the mainstream in nowadays AI industry is largely featured with the privatization of ML datasets, which are collected, sanitized, annotated and curated with a substantial amount of human and computing costs afforded by the data owner \cite{Wang2021AnnotationefficientDL}. As Bengio et al. stated in their Turing lecture, ``\textit{the availability of large datasets were key enablers of deep learning}'' \cite{Bengio2021DeepLF}, which explains why private datasets are usually viewed as a critical private asset for AI corporations. Moreover, with deep learning extending into mission-critical scenarios (e.g., autonomous vehicle and intelligent health) where almost no large-scale well-annotated dataset previously exists, the exclusive ownership of relevant private datasets can be a huge advantage for a corporation in the competitive market, which, in turn, incentivizes illegal piracy from potential attackers.   

According to our field study, we also observe many other corporations implement such an application-then-authorization way of managing ML datasets. An employee who is assigned with certain modeling task can directly apply to accessing the relevant private dataset. Meanwhile, depending on how the authorization is executed by the supervisors, such a mechanism can degrade to a logging mechanism instead of providing strict access control mechanism on engineers from accessing irrelevant ML datasets. C

To highlight the privacy risks of allowing unnecessary access to private datasets, we present a novel insider attack called Matryoshka, which for the first time realizes the covert transmission of multiple secret DNNs (i.e., \textit{secret models}) via one scheduled-to-publish DNN (i.e., a \textit{carrier model}), for the purpose of stealing the functionality and the sensitive information of private dataset(s). Below, we first introduce the security settings of Matryoshka, and present an overview of our attack pipeline.  

Based on a novel weight sharing mechanism which allows us to covertly transmit multiple secret models in one published DNN, we propose the Matryoshka attack to break the privacy barrier of ML datasets even with no exposed interfaces.


Intuitively, with the above primitives, a ParamPool can be used as a proxy to the full life cycle of a DNN. Before detailing the implementation and the usage of the above primitives, we first introduce the pipeline of our attack.    


The attacker creates a ParamPool \textit{from scratch} with a customized size for each parameter group. To simulate the parameters in a normal DNN, the parameters in the weight group $\mathcal{P}_w$ are initialized from a Gaussian distribution, the parameters in the bias group are initialized as $0$, while the parameters in the scale group are initialized as $1$. \textit{(Option II)} The attacker collects and groups all the learnable parameters from the carrier DNN $C$ to form the ParamPool.

 in the following ways: \textit{(Option I)}.
 
     Option I implements a natural replication scheme if the size of ParamPool is times smaller than the carrier model. Consequently, the carrier model becomes more robust  In contrast, Option II is by design more advantageous in evading detection of hidden models, as the parameters of the carrier model contain no detectable composition patterns (e.g., repetitive values) and exhibit an indistinguishable distribution as a normally trained model after the hiding process .       
     
     
    \noindent$\bullet$ \textbf{Example} -- For a private dataset $D_k$ initially built for medical object detection \cite{pmlr-v116-jaeger20a}, the attacker can choose the secret model $f_k$ as a single shot multibox detector (SSD \cite{Liu2016SSDSS}) with MobileNetV2 \cite{Sandler2018MobileNetV2IR} as its backbone. Both the two architectures are well-referenced and can be replicated by a colluder who only knows the architecture names. The attacker may be required to preprocess the input images from the private dataset to stay compatible with the known architectures. According to the convention of object detection \cite{Liu2016SSDSS}, the loss function $\ell_k$ is implemented as the weighted sum of a localization loss (i.e., for location regression of the bounding box) and a confidence loss (i.e., for classification of the bounding box). For more background information, please refer to Appendix \ref{sec:appendix:dnn}.
    
    \noindent$\bullet$ \textbf{Example} -- For stealing the face images of a certain identity from a private dataset for face recognition, the attacker can instantiate the secret model $f_k$ as the generator  module in DCGAN \cite{Radford2016UnsupervisedRL}, a well-known fully convolutional architecture which is widely used in generative adversarial learning \cite{Goodfellow2014GenerativeAN}. For the detailed architecture, please refer to \S\ref{sec:appendix:dnn}. As in \cite{Radford2016UnsupervisedRL}, we choose the noise distribution $P_k$ as the standard multivariate Gaussian distribution, and measure the distance between the generated and the ground-truth input by the mean square error.    



 (shuffled by a random permutation specified with the integer secret $v_k$) which belongs to the same group of the original parameter. According to L4-14 in Algorithm \ref{alg:fill}, 
 
 As is introduced in \S\ref{sec:prelim:dl}, DNN is mostly composed of learnable parameters, which can be encoded and covertly transmitted by our ParamPool-based approach above. However, the class of batch normalization (i.e., BatchNorm \cite{Ioffe2015BatchNA}) layers is an exception. A self-contained introduction on BatchNorm is presented in Appendix \ref{sec:appendix:dnn}.  
 
 Specifically, the outsider can first forward all the training batch to the first BatchNorm layer, which accumulates the mean and the variance of the input features of the batches. According to the central limit theorem, if the batches are uniformly sampled, the estimated mean and variance on the random batches are effective estimators to the statistics on the whole training dataset.  Recursively, the warm-start process adjusts the non-learnable parameters until the last BatchNorm layer. 
 
  as when it finishes training on the private dataset
  
  For the model details, please refer to Appendix \ref{sec:appendix:exp}.
  
  %%%%%%%%%%%%% BEGIN OF PILOT STUDY RESULTS
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.45\textwidth]{img/defense.pdf}
\caption{}
\label{fig:defense}
\end{center}
\end{figure}
%%%%%%%%%%%%%% END OF PILOT STUDY RESULTS
 
%%%%%%%%%%%%% BEGIN OF Facescrub visualization
\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.45\textwidth]{img/facescrub_visualize.jpg}
\caption{Sampled results on Facescrub with different data stealing approaches.}
\label{fig:facescrub_visualization}
\end{center}
\end{figure}
%%%%%%%%%%%%%% END OF FaceScrub visualization

 This poses huge threats especially on datasets that contain sensitive information or constitute intellectual property rights. Below, we briefly review this fruitful branch according to the types of the revealed information. 

 In other words, with model extraction attacks, the adversary can craft a working model on the private dataset without actually accessing the dataset \cite{Tramr2016StealingML}.   
 
 To summarize, most existing privacy attacks on training data essentially exploit the high tension between the privacy of the training data and the openness of the ML models, which especially becomes a security risk for well-trained DNN because they tend to remember much more about the training data than we expect \cite{Carlini2021ExtractingTD}. 
 
 provides a novel perspective compared with existing privacy attacks and 
 
 , our proposed data stealing approach encodes much more data inputs by hiding generator-like models in the carrier model instead of hiding raw data. Compared with the data hiding approach, Matryoshka recovers the encoded inputs with almost no reconstruction error while almost no utility loss is incurred on the carrier model.   
 
  which may impair the cooperation's business strategy to some degree
  
  


\noindent\textbf{Choice of Attack Timing.} However, we admit that, as a common weakness of insider attacks \cite{kandias2013insider}, Matryoshka would be detected when the malicious code undergoes a thorough code review. This may happen when the task of training the carrier model $C$ is assigned as a team work. Nevertheless, the attacker can avoid such a risk by choosing a proper attack timing according to the nature of the assigned task. In fact, the capability of Matryoshka of hiding a large model in a much smaller one adds more flexibility to the timing choice. When the carrier model is less complicated, the more possible the task is assigned to an individual. Moreover, after the carrier model  is prepared, the attacker needs to clear all the traces about the attack (including codes, intermediate results, logs, etc.)  and only preserves the essential information and products when training a normal model for the assigned task.  

, and to explore potential mitigation approaches to eliminate the threats of Matryoshka

% For the first time, we show the possibility of exploiting such a model to hide and covertly transmit (i) task-oriented models trained on the private datasets for functionality stealing or (ii) memorization-oriented models for sensitive data stealing. 
the adversary has no access to a training dataset which caters for his/her requirement. 

From the pay-per-query prediction APIs on ML-as-a-Service platforms (e.g., Amazon AWS \cite{amazon_aws}) to the freely available models on third-party model zoos (e.g., Apple Developer \cite{torch_hub}), well-trained DNN models tend to remember too much about the private training data. 

\textbf{``\textit{The availability of large datasets are key enablers of deep learning}'', as stated by Bengio et al. in the Turing lecture \cite{Bengio2021DeepLF}. }





have access to the local network of the data center but are strictly forbidden from invoking data transmission to the outside due to typical data security models deployed in IT corporations  (\S\ref{sec:data_security_study}). Yet, confined to the local network, an insider still have multiple ways to access the private dataset, e.g, when he/she is assigned with workloads related to the private dataset or applies to access the private dataset for, e.g., \textit{multimodal learning} (i.e., a learning paradigm which leverages multiple datasets from different domains to enhance the model training \cite{Baltruaitis2019MultimodalML}). Our work for the first time shows, only if such an insider is also assigned with a task of training an independent DNN model on an irrelevant non-target dataset which later undergoes a model publishing process  \cite{google_bert,openai_git}, he/she can cause severe leakage of the functionality and the sensitive information from almost any private dataset with no public interface.             

 \footnote{By convention, Matryoshka dolls inside (i.e., the secret models) is more precious than the outer doll which holds them (i.e. the carrier model).}
 
 (e.g., over $10$ millions parameters are contained in a ResNet-18 \cite{He2016DeepRL} trained for ImageNet classification \cite{Deng2009ImageNetAL})
 
 and can hide a diversity of DNN models in the carrier model during its construction 
 
 Meanwhile, almost no utility loss ($< 1\%$) is incurred compared with a normally trained model.IN popular data security models in AI corporations, almost any DNN engineer can be a potential Matryoshka attacker who has access to the target private dataset(s) and is responsible for using an irrelevant dataset to train an independent scheduled-to-publish model (i.e., the \textit{carrier} model).
 

In the former case, the adversary targets at the most sensitive data inputs contained in the private training data. For example, a recent line of works reveal and evaluate how sensitive texts (e.g., social security number) are memorized in DNN-based online services \cite{Carlini2019TheSS} (e.g., Google's Smart Compose \cite{Chen2019GmailSC}) and more recent industry-level pretrained large language models \cite{Carlini2021ExtractingTD} (e.g., OpenAI's GPT-2 \cite{Radford2019LanguageMA}).


 or (ii) memorization-oriented models (of a generator-like DNN architecture \cite{Goodfellow2014GenerativeAN,Radford2016UnsupervisedRL}, which maps random noises to real data samples) for sensitive data stealing. 
 
 In unsupervised learning tasks, a fundamental goal is to learn the distribution of the input data in $\mathcal{X}$ with either parametric or non-parametric models. For example, in the branch of generative adversarial nets (GAN \cite{Goodfellow2014GenerativeAN}), a parametric generative model $g(Z;\theta)\in\mathcal{X}$ is trained to map a random variable $Z \sim \mathcal{N}(0, \sigma^2)$, i.e., a fixed Gaussian distribution, to fit the true data distribution supported at $\mathcal{X}$.

==> tex/tables/dataset_archi.tex <==
\begin{table}[H]
\centering
\caption{Datasets and architectures.}
\label{tab:datasets}
\scalebox{0.8}{
\begin{tabular}{lll}
\toprule
Dataset & Task & Architecture \\
\midrule
CIFAR-10 \cite{krizhevsky2009learning}& Object Classification & ResNet-18 \cite{he2016deep} \\
GTSRB \cite{Houben-IJCNN-2013} & Traffic Sign Recognition & VGG-16 \cite{simonyan2014very}\\
DermaMNIST \cite{medmnistv2}& Skin Cancer Diagnosis & LeNet-5\cite{lecun1998gradient}\\
IMDB \cite{maas-EtAl:2011:ACL-HLT2011}& Sentiment Classification & TextCNN \cite{zhang2015sensitivity}\\
SpeechCommand \cite{speechcommandsv2} &Speech Recognition&M5 \cite{7952190}\\
Warfarin \cite{Truda2020warfit}& Dose Estimation&MLP \\
VOC'07 \cite{Everingham15}& Object Detection &MoblieNetV2-SSD\cite{howard2017mobilenets} \\
UWave \cite{liu2009uwave}& Time Series Classification &RNN \\
\bottomrule
\end{tabular}}
\end{table}

==> tex/tables/speechCommandStealing.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \label{speechcommand}
  \caption{The effectiveness of data stealing in terms of SpeechCommand}
    \begin{tabular}{ccc}
    \toprule
    \multirow{2}[4]{*}{\textbf{\# Inputs}} & \multicolumn{2}{c}{\textbf{Matryoshka}} \\
\cmidrule{2-3}          & MSE   & Acc \\
    \midrule
    256   & 0.000150028 & 95.15\% \\
    512   & 0.000269945 & 95.07\% \\
    1024  & 0.000350233 & 95.31\% \\
    2048  & 0.000424155 & 95.09\% \\
    4096  & 0.000488342 & 95.15\% \\
    \bottomrule
    \end{tabular}%
  \label{tab:speech}%
\end{table}%

